Asset Prices and Capital Share Risks: Theory and Evidence

An asset pricing model using long-run capital share growth risk has recently been found to successfully explain U.S. stock returns. Our paper adopts a recursive preference utility framework to derive an heterogeneous asset pricing model with capital share risks.While modeling capital share risks, we account for the elevated consumption volatility of high income stockholders. Capital risks have strong volatility effects in our recursive asset pricing model. Empirical evidence is presented in which capital share growth is also a source of risk for stock return volatility. We uncover contrasting unconditional and conditional asset pricing evidence for capital share risks.

==> chapters/4-Data-Priors/instr.tex <==
\subsection{Instrument Variables}
Event study


==> chapters/4-Data-Priors/projection.tex <==
\subsection{Factor Projection}
\noindent
%\textit{The Capital share factor is a macroeconomic term calculated by the capital}
In equation (\ref{eq:mfapm}), the Jensen's alpha of MFAPM is interpreted as an "abnormal" return. However, the capital share factor is not traded in the market, hence no actual return is associated with this factor.
As suggested by \cite{lamont2001economic}, values of nontraded factors should be projected into an excess return space to explain the Jensen's alpha properly. Following the projection method proposed by \cite{bianchi2017macroeconomic}, this paper projects capital share factor using the following equation:
\begin{equation}
    KS_t=a+b~x_t+c'~z_{t-1}+\epsilon_t ~~~~~~~~~~~~~~~~~~\epsilon_t\sim N(0,\omega)
    \label{eq:projection}
\end{equation}
`In equation (\ref{eq:projection}), $x_t$ represents excess returns of six zero-investment portfolios and $z_{t-1}$ represents three instruments capable to predict returns. The purpose of including instruments, also called control variables, is to close the gap between expected returns and real returns. \cite{lamont2001economic} shows that, in most cases, the effects of tracking portfolios constructed using different methods are similar. That is, the baseline portfolio is robust to different specifications. Hence, constructing particular tracking portfolios for capital share factor is unnecessary since the baseline portfolios are roughly the same. For the sake of consistency in non-traded factors projection by \cite{bianchi2017macroeconomic}, this paper selects same portfolios and instruments to span a large proportion of the return space. Portfolios include six equity net zero investment portfolios sorted by size and book-to-market ratio, term yield spreads of government bonds, and term yield spreads of corporate bonds. Instruments include lagged yield spread of long-term Treasury bonds minus the T-bill yield, credit yield spread of long-term corporate bonds and government bonds, and the lagged real short-term bill rate.
\smallbreak
The result mimicking portfolio of capital share factor is denoted by:
\begin{equation}
    FMP_t=\hat{a}+\hat{b}'~x_t 
    \label{eq:mimick}
\end{equation}
where the sum of $\hat{a}$ and $\hat{b}$ does not have a theoretical boundary because the portfolios for projection are all zero-investment portfolios \citep{lamont2001economic}.
\smallbreak
\begin{center}
    \textcolor{red}{I WANT TO LEAVE IT AFTER CRIEFF, OR IF I COULD HAVE TIME FOR IT. AS FOR THE EXTENSION OF DATA PERIOD, I THINK I DON'T HAVE TIME BEFORE CRIEFF}
\end{center}

==> chapters/Methodology/classification_problem.tex <==
\subsubsection{Hierarchical Shrinkage  Prior for "Redundant" Factors}
The noninformative prior, which is adopted by B-TVB-SV framework, leads to the risk loadings centered at the unrestricted least squares (LS) quantities \citep{korobilis2013hierarchical}. Classical Bayesian shrinkage priors have undesirable properties when the amount of risk factors are relatively large. For example, ridge regression prior is a global prior which assign same shrinkage level for all factors, while empirical Bayes priors and g-priors are highly relied on a precise estimation of information matrix \citep{korobilis2013hierarchical}. The hierarchical shrinkage prior only require a hyper-prior distribution for all elements in covariance matrix, of which the posterior can be used as priors for factor loadings.
\smallbreak
Under a time-varying parameter setting, \cite{huber2019inducing} estimates the forecasting performances of various Bayesian shrinkage priors, including a loosely informative prior (flat), the Dirichlet-Laplace prior (DL) , the Bayesian Lasso (Lasso), the Normal-Gamma prior (NG), the Horseshoe prior (HS), and the Normal-mixture of Inverse Gamma prior (NMIG). The time-varying parameter (TVP) model used by \cite{huber2019inducing} is similar as equations (\ref{eq:btvbsv1}) and equation (\ref{eq:tvb}):
\begin{equation}
    \beta_{ij,t}=\beta_{ij,t-1}+w_{ij,t}
    \label{eq:huber_beta}
\end{equation}
The $w_{ij,t}$ term is assumed to follow a random walk with $w_{ij,t}\sim N(0_K,V)$, where $V=diag(v_{ij},...,v_{iK})$ is the variance-covariance  matrix of state innovations and $\upsilon_{ij}$ is a process innovation variance of the $i^{th}$ excess return associated with the $j^{th}$ factor loading. In this paper, as stated in equation (\ref{eq:tvb}) and equation (\ref{eq:pi}), $\kappa_{ij,t}\eta_{ij,t}$ term follows a mixture of normal distribution when $\kappa_{ij,t}=1$ with probability  $\pi_{ij}$ and, a point distribution when $\kappa_{ij,t}=0$ with probability $1-\pi_{ij}$. When the break probability of $\kappa_{ij,t}$ equals to one, the model in this paper is consistent with the model proposed by \cite{huber2019inducing}, while when $\pi_{ij}$ equals to zero, the $\beta_{ij,t}$ becomes a constant. Therefore, this paper consider the TVP model with structure breaks as a classification problem between a TVP model or a static model. In the case when $\kappa_{ij,t}=1$, equation (\ref{eq:tvb}) is identical to equation (\ref{eq:huber_beta}), and the non-centered parameterization of equation (\ref{eq:btvbsv1}) is as follows \citep{huber2019inducing}:
\begin{align}
        & r_{i,t}=\alpha_{i0,t}+\sum^2_{j=1}\beta_{ij,t}F_{j,t}+\sum^ {K}_{j=3}\Tilde{\beta}_{ij,0}F_{j,t}+\sum^ {K}_{j=3}\Tilde{\beta}_{ij,t}\sqrt{v_{ij}}F_{j,t}+\sigma_{i,t}\epsilon_{i,t}~~~~~~~~~~~\epsilon_{i,t}\sim N(0,1)\label{eq:nonpara}\\
        & \Tilde{\beta}_{ij,t}=\Tilde{\beta}_{ij,t-1}+\Delta_{ij,t}  ~~~~~~~~~~~\Delta_{ij,t}\sim N(0,1) \label{eq:nonpara_b}
\end{align}
where the time-varying parameters is modified as  $\Tilde{\beta}_{ij,t}=\frac{\beta_{ij,t}-\beta_{ij,0}}{\sqrt{v_{ij}}}$ to ensure normal distributed error terms $\Delta_{ij,t}$. Notice that the factor loadings subjected to shrinkage are identified manually in this paper. In econometric studies, a principal component model is usually used as a benchmark for the number of variables subject to shrinkage. Instead of using the econometric way, this paper adopts the theoretical guidance stated in equation (\ref{eq:ks_apx}) as a benchmark for factor shrinkage. 
\smallbreak
The equation (\ref{eq:nonpara}) can be written as:
\begin{equation}
     r_{i,t}=\alpha_{i0,t}+\sum^2_{j=1}\beta_{ij,t}F_{j,t}+\sum^ {K}_{j=3}\Tilde{\beta}_{ij,0}F_{j,t}+\sum^ {K}_{j=3}\sqrt{v_{ij}}Z_{j,t}+\sigma_{i,t}\epsilon_{i,t}~~~~~~~~~~~\epsilon_{i,t}\sim N(0,1)
     \label{eq:shrinkage_z}
\end{equation}

\cite{huber2019inducing} find that when the number of regressor is small, the sparsification tend to be more important than shrinkage. Hence, the flat prior outperforms other priors in the case which is similar as this paper: moderate sparse level (70\% true values of coefficients are zeros, theoretically 80\% in this paper), 15 independent variables (10 factors in this paper) and 400 observations ($T=360$ in this paper).  Global-local shrinkage priors, such as HS, are not necessary to be tested by this paper. Global-local shrinkage priors perform better than flat prior when the model involves a large number of variable , while the MFAPM model of interest only contains 10 factors with no lags.
%\textcolor{red}{IF HAVE TIME: However, NG outperforms other priors in the case with a denser DGP (30\% true values of coefficients are zeros) holding other conditions equal and Flat prior performs badly under this setting. THEN compare flat and NG. (NG is global-local so delete the following sentence)} 
%Therefore, this paper choose HS as the shrinkage prior due to its attractive theoretical properties: the robustness of estimation under and the ability to capture various patterns.

%Adaptive shrinkage Jeffreys’ prior, Adaptive shrinkage t-priors, Hierarchical LASSO, Hierarchical fused LASSO, Hierarchical elastic net and DFM. 

\smallbreak
As suggested by \cite{huber2019inducing}, and \cite{ray2018signal}, this paper adopts the Signal Adaptive Variable Selector (SAVS) algorithm to estimate the factor loading shrinkage. The SAVS algorithm is developed to solve the problem that hierarchical shrinkage priors do not shrink the noise coefficients exactly to zero.
 According to equation (\ref{eq:shrinkage_z}), the SAVS estimator has the following form when structural breaks present in factor loadings:
\begin{equation}
    \sqrt{\hat{v}^*_{ij}}=sign(\sqrt{\hat{v}_{ij}})||Z_{j,t}||^{-2}(\sqrt{\hat{v}_{ij}}\cdot ||Z_{j,t}||^2-\mu^\upsilon_{ij})_+~~~~~~~~~~~j=3,...,K
    \label{eq:savs_tvp_beta}
\end{equation}
where $\mu^\upsilon_{ij}=\frac{1}{\hat{v}_{ij}}$ and $\sqrt{\hat{v}_{ij}}$ denotes the posterior mean of $\sqrt{v_{ij}}$.
%forward-filtering backward-sampling algorithm proposed in Carter and Kohn (1994) and Fr¨uhwirth-Schnatter (1994).\\

 In the case when $\kappa_{ij,t}=0$, factor loadings are constant. Therefore, this paper uses  estimated factor loadings $\hat{\beta}_{ij,t}$ and factors $F_{ij,t}$ directly to obtain the SAVS estimator $\hat{\beta}^*_{ij,t}$ for $j=3,...,K$.
 The SAVS estimator has the following form when factor loadings are constant:
\begin{equation}
    \hat{\beta}^*_{ij,t}=sign(\hat{\beta}_{ij,t})||F_{j,t}||^{-2}(|\hat{\beta}_{ij,t}|\cdot ||F_{j,t}||^2-\mu^\beta_{ij})_+~~~~~~~~~~~j=3,...,K
    \label{eq:savs_constant_beta}
\end{equation}
where $\mu^\upsilon_{ij}=\frac{1}{\hat{\beta}^2_{ij}}$ and $\hat{\beta}_{ij,t}$ denotes the posterior mean of $\beta_{ij,t}$.
In the new algorithm based on SAVS, the $\kappa_{ij,t}$ included as the indicator for structural breaks. The factor loadings are categorised by calculating $\beta^1_{ij,t}=\kappa_{ij,t}\beta_{ij,t}$ and $\beta^2_{ij,t}=(1-\kappa_{ij,t})\beta_{ij,t}$: in the $\beta^1_{ij,t}$ group, all factor loading posteriors are identical to factor loading posteriors estimated by a TVP model; in the $\beta^2_{ij,t}$ group, all factor loading posteriors are identical to factor loading posteriors estimated by a static model. After the classification of posteriors, this paper applies SAVS algorithm differently to $\beta^1_{ij,t}$ and $\beta^2_{ij,t}$, as stated by equation (\ref{eq:savs_tvp_beta}) and equation (\ref{eq:savs_constant_beta}) respectively.  
\smallbreak
\textcolor{red}{the following is my new algorithm}
\lstinputlisting[language=Octave]{reports/shrinkagereport.m}

==> chapters/Results/vrp.tex <==
\section{Capital Share Growth and Variance Risk Premium}
Quantitatively, the capital share factor might have long-run correlation with the latent variance risk premium (VRP) variable. The VRP is also based upon \cite{epstein1989substitution} utility function and is a relatively new topic in asset pricing (see \cite{stein1991stock}, \cite{kilic2019good}, \cite{ferson2019empirical}, etc.), and is defined as the difference between the risk neutral expectation and the objective expectation of the return variation \citep{zhou2018variance}. In existing literatures, economic uncertainty can be proxied by the VRP which correlates negatively with future macroeconomic performance \citep{bali2016risk}. VRP is introduced to price equity returns and is shown to have high correlation with proxies of uncertainties associate with macroeconomics, return distribution of financial firms, CDS market and disagreement about individual stocks \citep{bali2016risk}. 

The implication of VRP is based on a consumption-based asset pricing model. Although the economic model motivates the VRP assumes homogeneous agents in the market and a Lucas Tree endowment (see \cite{kilic2019good}), the VRP enters the general equilibrium equation as an uncertainty variable. The inequality and redistribution risks potentially explain the consumption uncertainty in this general equilibrium model, thus might be sources to generate VRP. The VRP in the market is not directly observable \citep{zhou2018variance}. Therefore, literatures construct proxy, namely VRP factor, to represent VRP using uncertain approach which relies on the nonstandard recursive utility framework \cite{zhou2018variance}. The construction of the VRP factor is usually data-based: the VRP factor is calculated by the implied risk minus the model-free realized risk using high frequency (5-minute) data (see \cite{kilic2019good}, \cite{zhou2018variance}, and \cite{bali2016risk}). The implied risk is derived by a portfolio of European calls, basing upon Black-Scholes model which does not assume homogeneous consumers. The realized risk is the difference between squared positive returns and squared negative returns. Therefore, the construction of VRP is not conflict with the inequality-based assumption which motivates the capital share factor. 
 
This paper adopts the VRP factor constructed by \cite{kilic2019good} to derive quantitative evidences for the relationship between the capital share factor and the VRP factor. The VRP factor is constructed using
5-minute S&P 500 futures returns and S&P 500 index options. The sample of VRP factor adopted by this paper spans 1988 January to 2014 August. According to equation (\ref{eq:price_kernel}) and the construction of VRP, the squared capital share factor should be correlated with VRP. This paper regresses the demeaned capital share factor on the demeaned VRP factor using a simple Ordinary Least Square (OLS) regression.  For the OLS estimate of squared capital share factor on VRP, the coefficient is expected to be significant for factors which captures the true DGP of portfolio returns but insignificant under B-TVB-SV approach. The VRP is positively correlated with excess equity returns because it serves as a compensation of consumption uncertainty \citep{zhou2018variance}. The capital share factor captures the redistribution risks and is found to have positive risk premium by \cite{lettau2019capital}. Therefore, the two variables should be positively correlated if they capture the same market risk component. As shown by Figure \ref{fig:vrp}, the variance of VRP factor is generally higher than factors tested in this paper because that the construction of VRP factor is based upon cumulative outcomes of squared high frequency data. Therefore, the $R^2$ estimates are expected to be relatively low, and this paper only focus on the partial effect indicated by statistics associated with coefficients.
\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{chapters/figures/vrp.jpg}
        \caption{\textbf{Variance risk premium (\%).} VRP data is obtained from \cite{kilic2019good} directly. Sample of the VRP factor spans 1988 January to 2014 August.}
    \label{fig:vrp}
\end{figure}
Table \ref{tab:vrp} reports OLS estimates of squared capital share factor on VRP factor. In this table, the coefficient of squared capital share factor is positive and significant at 5\% level, with a very high t-statistic of 6.450. According to results derived in this section, the squared capital share factor could serve as a potential substitution of VRP factor. Thus, the risk premiums generated by excess volatility could be explained as a consequence of volatility spillover from high income group to the whole equity market. 
\begin{table}[H]
\centering
\caption{OLS regression of capital share factor on VRP}
\begin{tabular}{@{}lccccc@{}}
\toprule
               &Coeff.&Std.err&t-statistic &p-value &$R^2$(\%)   \\ \midrule
  $F^2_{KS}$ & 9.433**  & 1.463& 6.450& 0.000& 11.289    
    \\ \bottomrule
\end{tabular}
\\
\begin{tablenotes}
OLS estimates of squared capital share factor on VRP factor. Data used is demeaned and of percentage scale. ** denotes the estimate is significant at 5\% level. * denotes the estimate is significant at 10\% level. Sample spans 1988 January to 2014 August.
\end{tablenotes}
\label{tab:vrp}
\end{table}


%Combining equation (\ref{eq:mfapm_kssigma}) and equation (\ref{eq:garch}), the equity returns can be written as 
%\begin{equation}
%    r_{i,t}=\beta_{i0,t}+\beta_{iC,t}(\frac{C_{t+1}}{C_{t}})+\beta_{i\sigma,t}(\sigma^2_{i,t-1}+\gamma^2_{KS,t} F^2_{KS,t}+2\gamma_{KS,t}\sigma_{i,t-1} F_{KS,t})+\epsilon_{i,t}
%\end{equation}
%If the DGP in equation (\ref{eq:mfapm_kssigma}) holds, the factor loadings of $F_{KS}$ and $F^2_{KS}$ are expected to be partially correlated.
%Secondly, this paper adopts the variance equation similar as specified by \cite{bianchi2017macroeconomic} in equation (\ref{eq:sv}) for sanity check of the impact of the capital share factor on return volatilities. Instead of estimating a single capital share factor model, this paper estimates the size/BM sorted portfolios by the capital share factor as follows: firstly, this paper regresses portfolio returns on a constant, and obtain the residuals for each portfolio; secondly, the residuals are squared to obtain the variance $\sigma^2$; finally, this paper regress the $ln(\sigma^2_t)$ on its lag and the capital share factor. The regression results are reported in Table \ref{rab:garch_check} (see Appendix). As shown by this table, most of coefficients of the capital share factor are significant. For some portfolios, such as ME3B1, ME5BM4, and BIGHiBM, the capital share factor explains the variation of $ln(\sigma^2_t)$ while the $ln(\sigma^2_{t-1})$ is insignificant. 


%The intuition behind the impact of capital share factor on market volatility is simple. At time $t-1$ and $t$, labour income does not change due to the fixed population size and the sticky wage within a short time horizon, say one month. \textcolor{red}{Conditional on the assumption derived by \cite{lettau2019capital} of the stylized economy holds, there is no switch between the population consuming capital income and the population consuming labour income and the participation rate of stock market does not change. Therefore, in this case, the capital share growth measures the growth of the total capital income to total wage income ratio in the economy. The demand and supply relationship within the stock market is not affected by changes of the capital share, but the total capital market value is positively correlated with the capital share growth. Therefore, the financial leverage and operating leverage is increased, leading to a higher market volatility \citep{binder2001stock}. In the economy, as evidence shown by \cite{lettau2019capital}, the capital share has strong positive correlation with the income share of the individuals on the top decile wealth distribution, but has negative correlation with the rest. The growth of aggregate consumption is also found to be more volatile on the top of the wealth distribution compared to that on the bottom \cite{lettau2019capital}. Therefore, the positive capital share growth increases the difference between the income shares of top and bottom individuals in the wealth distribution, and increases the proportion of consumption which grows with a higher volatility.2   }

%\textcolor{blue}{In reality, the all individuals in the economy have access to the stock market. The capital share growth is positively correlated with the participation rates of stock market. Therefore, the positive growth indirectly shows that a fraction of population shifts from labour workers to stock market participants, but this fraction of population is not sophisticated as experienced investors. Therefore, the growth of capital share increases the diversity of information and decision making strategies in the stock market, and brings about a higher volatility in portfolio returns. Meanwhile, a higher stock market participation rate also indicates that the overall risk tolerance level increases for the population, thus the required subsidy for investors to bear risks decreases. Although the demand of stocks increases as the capital share grows higher, the risk tolerant level of investors also increases, thus the capital share factor has insignificant effects on the mean equation of portfolio returns. }


==> chapters/Results/vrp_notes.tex <==
The good and bad variance premiums proposed by \cite{kilic2019good} have good performance in predicting asset returns. Therefore, this paper adopt these two factors to investigate the relationship between capital share factor and the upside and downside risk in financial market. In Table \ref{tab:btvbsv_lambda_single}, the difference between the average and the median are positive. Although the risk premiums are slightly skewed right and some return distribution properties have explanatory power, this paper does not study the effect of skewness or kurtosis of the capital share factor. The skewness and kurtosis are found to be materially neutral for the signs and magnitudes of risk premium estimates when including the good and the bad variance premium factors \citep{kilic2019good}. The good and bad realized variance are constructed as follows \cite{kilic2019good}:
\begin{equation}
    rv^g_t=\sum^{H_t}_{i=1}r^2_{i,t}I(r_{i,t}>0)
    \label{eq:rv_g}
\end{equation}
\begin{equation}
    rv^b_t=\sum^{H_t}_{i=1}r^2_{i,t}I(r_{i,t}\leq0)
    \label{eq:rv_b}
\end{equation}
Equation (\ref{eq:rv_g}) and equation (\ref{eq:rv_b}) denotes the construction methods of the good realized variance and the bad realized variance respectively. The $H_t$ term is the 
\smallbreak
The construction of the good or the bad variance premiums involves high frequent data such as daily. However,  

\textcolor{red}{We use 5-minute S&P 500 futures returns from TICKDATA to construct the realized variance measures at a monthly frequency}
\textcolor{red}{ks only correlate with downside risk not the difference; ff3 correlate with the upside-downside}

==> chapters/equitypuzzle.tex <==
\subection{Rolling-window Multiplicative GARCH}
Capital share factor can also be employed as an example justifying that the level effect and volatility effect should be considered separately when testing risk factors. Notice that, in Section \ref{section:theory}, capital share factor is also found to enter the volatility of consumption growth. This paper further consider the potential explanation of the equity pricing puzzle: the inability of standard CCAPMs to rationalize the statistics of equity returns. Due to the factor that the level effect and the volatility effect are pooled together in most of F-MB type estimation methods, the risk premium estimates of factors might become insignificant when the level effect and the volatility effect cancel each other. The bootstrap  procedure could solve such type of problem to some extent, but this paper doubt the capability of re-sampling approaches on ruling out the volatility effect completely.

This paper propose an alternative perspective: according to theoretical justifications, the variance equation is modeled explicitly. As shown by the DGP in equation (\ref{eq:mfapm_kssigma}), the consumption growth rate should have significant level effect when including capital share factor in the variance equation.  Following \cite{parker2005consumption}, the consumption growth factor is constructed using long-term consumption growth to avoid measurement error.  According to equation (\ref{eq:log_g_apx}), this paper uses 12-month consumption growth to maintain the consistency with the capital share factor. 

To test the SDF in equation (\ref{eq:sdf_garch}), the B-TVB-SV approach of a parsimonious consumption growth factor model is employed as a benchmark for the robust estimation of level effect. This paper then estimates a multiplicative GARCH(1,1) model in which the consumption growth factor enters the mean equation, and the variance equation is identical to equation (\ref{eq:garch2}). 

\begin{table}[ht]
\centering
\caption{Estimation of the new SDF}
\begin{tabular}{@{}lcccc@{}}
\toprule
                   & size/BM & REV & size/INV & size/OP \\ \midrule
                   &\multicolumn{4}{c}{Panel A: Bootstrap F-MB estimation}\\
$\beta_0$       & 0.459**        & 1.143**    & 1.293**        & 1.276**         \\
                &(0.006)&(0.006)&(0.000)&(0.000)\\
$Cons.growth$   &0.279         &-0.055     &-0.292         & -0.282**         \\
                &(0.142)&(0.308)&(0.641)&(0.654)\\\midrule                   
                   &\multicolumn{4}{c}{Panel B: multiplicative GARCH(1,1) estimation }\\
                   &\multicolumn{4}{c}{Mean equation}\\
$\beta_0$       & 1.310**        & 1.143**    & 1.293**        & 1.276**         \\
                &(0.000)&(0.000)&(0.000)&(0.000)\\
$Cons.growth$        &-0.015         &-0.055     &-0.292         & -0.282**         \\
                &(0.810)&(0.308)&(0.641)&(0.654)
                   \\\bottomrule
\end{tabular}\\
\begin{tablenotes}
This table reports test estimates(\%) of the SDF in equation \ref{eq:sdf_garch} Panel A reports the simple OLS estimates, and Panel B reports multiplicative GARCH(1,1) estimates. Estimates in this table use average returns of 25 size/BM, 10 REV, 25 size/INV, and 25 size/OP sorted portfolios. P-values are reported in brackets below estimates. ** denotes the estimate is significant at 5\% level. * denotes the estimate is significant at 10\% level. Data are monthly data spans 1964 January to 2018 August.
\end{tablenotes}
\label{tab:garch_newsdf}
\end{table}
\begin{table}[h]
\centering
\caption{B-TVB-SV risk premium estimates.}
\begin{threeparttable}
\begin{tabular}{@{}lccccccc@{}}
\toprule\midrule
         & Average    & Std.err    & t-stat    & p-value    & 2.5\%    & 50\%   & 97.5\%   \\ \midrule
         & \multicolumn{7}{c}{Panel A: consumption growth factor model}\\
$\alpha$ & 1.208& 0.214&        5.648&        0.000&       -9.213&        1.475 &       9.612 \\
Cons.growth  & -0.838**&        0.272 &      -3.079 &       0.002 &      -13.46 &      -0.175 & 8.823 \\ \bottomrule
\end{tabular}\\
\begin{tablenotes}
 Risk premiums in this table are estimated by a single capital share factor model using 25 size/BM sorted portfolios. Data used are monthly data from 1964 January to 2018 August. The first 10-year data are used as training sample for hyperparameter estimation, and the sample used for estimation spans 1974 January to 2018 August.
\end{tablenotes}
 \end{threeparttable}
     \label{tab:btvbsv_lambda_control}
\end{table}



==> chapters/shrinkage/lambdasavs.tex <==
\subsubsection{Hierarchical Shrinkage  Prior for "Redundant" Factors}
The noninformative prior, which is adopted by B-TVB-SV framework, leads to the risk loadings centered at the unrestricted least squares (LS) quantities \citep{korobilis2013hierarchical}. Classical Bayesian shrinkage priors have undesirable properties when the amount of risk factors are relatively large. For example, ridge regression prior is a global prior which assign same shrinkage level for all factors, while empirical Bayes priors and g-priors are highly relied on a precise estimation of information matrix \citep{korobilis2013hierarchical}. The hierarchical shrinkage prior only require a hyper-prior distribution for all elements in covariance matrix, of which the posterior can be used as priors for factor loadings.
\smallbreak
Under a time-varying parameter setting, \cite{huber2019inducing} estimates the forecasting performances of various Bayesian shrinkage priors, including a loosely informative prior (flat), the Dirichlet-Laplace prior (DL) , the Bayesian Lasso (Lasso), the Normal-Gamma prior (NG), the Horseshoe prior (HS), and the Normal-mixture of Inverse Gamma prior (NMIG). \cite{huber2019inducing} find that when the number of regressor is small, the sparsification tend to be more important than shrinkage. Hence, the flat prior outperforms other priors in the case which is similar as this paper: moderate sparse level (70\% true values of coefficients are zeros, theoretically 80\% in this paper), 15 independent variables (10 factors in this paper) and 400 observations ($T=360$ in this paper).  Global-local shrinkage priors, such as HS, are not necessary to be tested by this paper. Global-local shrinkage priors perform better than flat prior when the model involves a large number of variable , while the MFAPM model of interest only contains 10 factors with no lags.
\smallbreak
As suggested by \cite{huber2019inducing}, and \cite{ray2018signal}, this paper adopts the Signal Adaptive Variable Selector (SAVS) algorithm to estimate the factor loading shrinkage. The SAVS algorithm is developed to solve the problem that hierarchical shrinkage priors do not shrink the noise coefficients exactly to zero. The original SAVS algorithm is motivated by the solution of an optimization problem \citep{ray2018signal}: 
\begin{equation}
    \hat{\beta}^*:=argmin_\beta\{\frac{1}{2}||X\hat{\beta}-X\beta||^2_2+\sum^p_{j=1}\mu_j|\beta_j| \}
    \label{eq:savs}
\end{equation}
which is aimed to find the sparse value $\hat{\beta}^*$, which is close to $\hat{\beta}$, to minimize the Euclidean distance between model fit ($X\hat{\beta}$) and the true value of observations ($X\beta$). In equation (\ref{eq:savs}), the $j^{th}$ regressor is subject to shrinkage. In this paper, the B-TVB-SV method estimate both equation (\ref{eq:btvbsv1}) and equation (\ref{eq:btvbsv2}) within each iteration. The direct shrinkage of factor loadings become hard due to the tight link between the time-series estimation and the cross-sectional estimation . According to F-MB two step approach, the risk premiums estimated by equation (\ref{eq:btvbsv2}) should be centered around the counterpart risk factor in equation (\ref{eq:btvbsv1}) if the model is correctly specified. Therefore, this paper modifies the SAVS algorithm to tackle the shrinkage problem associated with two-stage regressions.
The optimization problem in this paper is 
\begin{equation}
    \lambda^*:=argmin_\lambda\{\frac{1}{2}||\lambda\beta-F\beta||^2_2+\sum^p_{j=1}\mu_j|\lambda_j| \}
    \label{eq:2stage_savs}
\end{equation}
The new SAVS estimator of the risk premium of the $j^{th}$ factor has the following form:
\begin{equation}
    \lambda^*_{j,t}=sign(\lambda_{j,t})||\beta_{ij,t}||^{-2}(|\lambda_{j,t}|\cdot ||\beta_{ij,t}||^2-\mu^\lambda_{j})_+~~~~~~~~~~~j=3,...,K
    \label{eq:savs_constant_beta}
\end{equation}
where $\beta_{ij,t}$ is the posterior of risk loading of the $j^{th}$ factor associates with the $i^{th}$ asset. In the original SAVS estimator, \cite{ray2018signal} set $\mu^\lambda_{j}=\frac{1}{\hat{\lambda}}$, where $\hat{\lambda}$ denotes the posterior mean of risk premiums. Under B-TVB-SV framework, this paper set $\mu^\lambda_{j}=\frac{1}{|F^2_{j}|}$ because the risk factor is the theoretical mean of its risk premium if the model is correctly specified.
\smallbreak 
A pseudo-code is provided as Algorithm \ref{alg:savs}.

\begin{algorithm}[H]
\SetAlgoLined
\SetKwInOut{1}{Write here the result }
\textbf{Within each iteration $m$:}\\
\textbf{Input:} Posterior estimation $\lambda^m_{j,t}$ and posterior estimation $\beta^m_{ij,t}$
 \While{j= 1 to p }{
  $\mu^\lambda_{j}=\frac{1}{|F^2_{j}|}$\;
  \eIf{$\lambda^m_{j,t}\cdot||\beta^m_{ij,t}||<=\mu^\lambda_j$}{
   $\lambda^{m*}_{j,t}=F_{j,t}$\;
   }{
    $\lambda^{m*}_{j,t}=sign(\lambda^m_{j,t})||\beta^m_{ij,t}||^{-2}(|\lambda^m_{j,t}|\cdot ||\beta^m_{ij,t}||^2-\mu^\lambda_{j})_+$\;
   
  }
   Sample $\beta^{m*}_{ij,t}$ conditional on $\lambda^*_{j,t}$\;
 }
 \textbf{Output:} Sparse estimation $\lambda^{m*}_{j,t}$ and  $\beta^{m*}_{ij,t}$
 \caption{2-stage SAVS Algorithm}
 \label{alg:savs}
\end{algorithm}
\textcolor{red}{A note: the new algorithm this paper built is quiet harsh in shrinkage: if the estimated risk premiums are not close enough to the values of the associated risk factor, the algorithm will set them directly to zero; if the risk premiums are close enough, the algorithm will shrink them toward to the values of the associated risk factor. This algorithm cannot be applied to all of the factors simultaneously because of the potential data mining problem. It could be possible that the algorithm should get ride of the if condition and do shrinkage for all risk premiums because the shrinkage extent in the first several interactions might be very large.}

\smallbreak

==> chapters/shrinkage/savs.tex <==
\subsubsection{Hierarchical Shrinkage  Prior for "Redundant" Factors}
The noninformative prior, which is adopted by B-TVB-SV framework, leads to the risk loadings centered at the unrestricted least squares (LS) quantities \citep{korobilis2013hierarchical}. Classical Bayesian shrinkage priors have undesirable properties when the amount of risk factors are relatively large. For example, ridge regression prior is a global prior which assign same shrinkage level for all factors, while empirical Bayes priors and g-priors are highly relied on a precise estimation of information matrix \citep{korobilis2013hierarchical}. The hierarchical shrinkage prior only require a hyper-prior distribution for all elements in covariance matrix, of which the posterior can be used as priors for factor loadings.
\smallbreak
Under a time-varying parameter setting, \cite{huber2019inducing} estimates the forecasting performances of various Bayesian shrinkage priors, including a loosely informative prior (flat), the Dirichlet-Laplace prior (DL) , the Bayesian Lasso (Lasso), the Normal-Gamma prior (NG), the Horseshoe prior (HS), and the Normal-mixture of Inverse Gamma prior (NMIG). The time-varying parameter (TVP) model used by \cite{huber2019inducing} is similar as equations (\ref{eq:btvbsv1}) and equation (\ref{eq:tvb}):
\begin{equation}
    \beta_{ij,t}=\beta_{ij,t-1}+w_{ij,t}
    \label{eq:huber_beta}
\end{equation}
The $w_{ij,t}$ term is assumed to follow a random walk with $w_{ij,t}\sim N(0_K,V)$, where $V=diag(v_{ij},...,v_{iK})$ is the variance-covariance  matrix of state innovations and $\upsilon_{ij}$ is a process innovation variance of the $i^{th}$ excess return associated with the $j^{th}$ factor loading. In this paper, as stated in equation (\ref{eq:tvb}) and equation (\ref{eq:pi}), $\kappa_{ij,t}\eta_{ij,t}$ term follows a mixture of normal distribution when $\kappa_{ij,t}=1$ with probability  $\pi_{ij}$ and, a point distribution when $\kappa_{ij,t}=0$ with probability $1-\pi_{ij}$. When the break probability of $\kappa_{ij,t}$ equals to one, the model in this paper is consistent with the model proposed by \cite{huber2019inducing}, while when $\pi_{ij}$ equals to zero, the $\beta_{ij,t}$ becomes a constant. Therefore, this paper consider the TVP model with structure breaks as a classification problem between a TVP model or a static model. In the case when $\kappa_{ij,t}=1$, equation (\ref{eq:tvb}) is identical to equation (\ref{eq:huber_beta}), and the non-centered parameterization of equation (\ref{eq:btvbsv1}) is as follows \citep{huber2019inducing}:
\begin{align}
        & r_{i,t}=\alpha_{i,t}+\sum^2_{j=1}\beta_{ij,t}F_{j,t}+\sum^ {K}_{j=3}\Tilde{\beta}_{ij,0}F_{j,t}+\sum^ {K}_{j=3}\Tilde{\beta}_{ij,t}\sqrt{v_{ij}}F_{j,t}+\sigma_{i,t}\epsilon_{i,t}~~~~~~~~~~~\epsilon_{i,t}\sim N(0,1)\label{eq:nonpara}\\
        & \Tilde{\beta}_{ij,t}=\Tilde{\beta}_{ij,t-1}+\Delta_{ij,t}  ~~~~~~~~~~~\Delta_{ij,t}\sim N(0,1) \label{eq:nonpara_b}
\end{align}
where the time-varying parameters is modified as  $\Tilde{\beta}_{ij,t}=\frac{\beta_{ij,t}-\beta_{ij,0}}{\sqrt{v_{ij}}}$ to ensure normal distributed error terms $\Delta_{ij,t}$. Notice that the factor loadings subjected to shrinkage are identified manually in this paper. In econometric studies, a principal component model is usually used as a benchmark for the number of variables subject to shrinkage. Instead of using the econometric way, this paper adopts the theoretical guidance stated in equation (\ref{eq:ks_apx}) as a benchmark for factor shrinkage. 
\smallbreak
The equation (\ref{eq:nonpara}) can be written as:
\begin{equation}
     r_{i,t}=\alpha_{i,t}+\sum^2_{j=1}\beta_{ij,t}F_{j,t}+\sum^ {K}_{j=3}\Tilde{\beta}_{ij,0}F_{j,t}+\sum^ {K}_{j=3}\sqrt{v_{ij}}Z_{j,t}+\sigma_{i,t}\epsilon_{i,t}~~~~~~~~~~~\epsilon_{i,t}\sim N(0,1)
     \label{eq:shrinkage_z}
\end{equation}

\cite{huber2019inducing} find that when the number of regressor is small, the sparsification tend to be more important than shrinkage. Hence, the flat prior outperforms other priors in the case which is similar as this paper: moderate sparse level (70\% true values of coefficients are zeros, theoretically 80\% in this paper), 15 independent variables (10 factors in this paper) and 400 observations ($T=360$ in this paper).  Global-local shrinkage priors, such as HS prior, are not necessary to be tested by this paper. Global-local shrinkage priors perform better than flat prior when the model involves a large number of variable , while the MFAPM model of interest only contains 10 factors with no lags.
%\textcolor{red}{IF HAVE TIME: However, NG outperforms other priors in the case with a denser DGP (30\% true values of coefficients are zeros) holding other conditions equal and Flat prior performs badly under this setting. THEN compare flat and NG. (NG is global-local so delete the following sentence)} 
%Therefore, this paper choose HS as the shrinkage prior due to its attractive theoretical properties: the robustness of estimation under and the ability to capture various patterns.

%Adaptive shrinkage Jeffreys’ prior, Adaptive shrinkage t-priors, Hierarchical LASSO, Hierarchical fused LASSO, Hierarchical elastic net and DFM. 

\smallbreak
As suggested by \cite{huber2019inducing}, and \cite{ray2018signal}, this paper adopts the Signal Adaptive Variable Selector (SAVS) algorithm to estimate the factor loading shrinkage. The SAVS algorithm is developed to solve the problem that hierarchical shrinkage priors do not shrink the noise coefficients exactly to zero. According to equation (\ref{eq:shrinkage_z}), the SAVS estimator has the following form when structural breaks present in factor loadings:
\begin{equation}
    \sqrt{\hat{v}^*_{ij}}=sign(\sqrt{\hat{v}_{ij}})||Z_{j,t}||^{-2}(\sqrt{\hat{v}_{ij}}\cdot ||Z_{j,t}||^2-\mu^\upsilon_{ij})_+~~~~~~~~~~~j=3,...,K
    \label{eq:savs_tvp_beta}
\end{equation}
where $\mu^\upsilon_{ij}=\frac{1}{\hat{v}_{ij}}$ and $\sqrt{\hat{v}_{ij}}$ denotes the posterior mean of $\sqrt{v_{ij}}$.
%forward-filtering backward-sampling algorithm proposed in Carter and Kohn (1994) and Fr¨uhwirth-Schnatter (1994).\\

 In the case when $\kappa_{ij,t}=0$, factor loadings are constant. Therefore, this paper uses  estimated factor loadings $\hat{\beta}_{ij,t}$ and factors $F_{ij,t}$ directly to obtain the SAVS estimator $\hat{\beta}^*_{ij,t}$ for $j=3,...,K$.
 The SAVS estimator has the following form when factor loadings are constant:
\begin{equation}
    \hat{\beta}^*_{ij,t}=sign(\hat{\beta}_{ij,t})||F_{j,t}||^{-2}(|\hat{\beta}_{ij,t}|\cdot ||F_{j,t}||^2-\mu^\beta_{ij})_+~~~~~~~~~~~j=3,...,K
    \label{eq:savs_constant_beta}
\end{equation}
where $\mu^\upsilon_{ij}=\frac{1}{\hat{\beta}^2_{ij}}$ and $\hat{\beta}_{ij,t}$ denotes the posterior mean of $\beta_{ij,t}$.
In the new algorithm based on SAVS, the $\kappa_{ij,t}$ included as the indicator for structural breaks. The factor loadings are categorised by calculating $\beta^1_{ij,t}=\kappa_{ij,t}\beta_{ij,t}$ and $\beta^2_{ij,t}=(1-\kappa_{ij,t})\beta_{ij,t}$: in the $\beta^1_{ij,t}$ group, all factor loading posteriors are identical to factor loading posteriors estimated by a TVP model; in the $\beta^2_{ij,t}$ group, all factor loading posteriors are identical to factor loading posteriors estimated by a static model. After the classification of posteriors, this paper applies SAVS algorithm differently to $\beta^1_{ij,t}$ and $\beta^2_{ij,t}$, as stated by equation (\ref{eq:savs_tvp_beta}) and equation (\ref{eq:savs_constant_beta}) respectively.  
\smallbreak
The property of Euclidean norm in equation (\ref{eq:savs_tvp_beta}) and equation (\ref{eq:savs_constant_beta}) supports the application of the classification approach: to classify the factor loadings into two different groups, this paper multiplies the coefficient matrix by the matrix containing all breaks. Let the matrix $I_\kappa$ denote the matrix containing all $\kappa_{ij,t}$. According to the properties of Euclidean norm, the equation $||I_\kappa Z||=|I_\kappa|\cdot||Z||$ and $||I_\kappa F||=|I_\kappa|\cdot||F||$ hold. Therefore, the multiplication of another matrix will not effect the properties of SAVS algorithm if the associated norms are all divided by $|I_\kappa|$ during the selection process. The equation (\ref{eq:savs_tvp_beta}) and equation (\ref{eq:savs_constant_beta}) will hold the same form after modification by $I_\kappa$.



==> chapters/shrinkage/shrinkage.tex <==
\section{Variable Selection and Shrinkage}
\cite{bianchi2017macroeconomic} tested a MFAPM including 9 factors and an intersection under the B-TVB-SV framework. Factors included in the 9-factor B-TVB-SV model are: the excess return of a value weighted market portfolio (MKT), the default risk premium change(DEF), the unexpected inflation rate(UI), the change in term premium (TERM), the industrial production (IP), the rate of real personal consumption growth (PC), the 1-month real T-bill return (T-bill), Liquidity factor (LIQ) and the Bond premium factor (BPF). Factor selected capture the macroeconomics risks (\cite{bianchi2017macroeconomic}).
\smallbreak
However, comparing equation (\ref{eq:sdf_factor}) and equation (\ref{eq:ks_apx}), if the inequality based CAPM holds, the core factors in SDF are the real consumption growth and the capital share growth. \cite{campbell1996understanding} also argues that, instead of simply selecting important macroeconomic variables, ICAPMs should select factors which can reflect the state variables related to future investment opportunities.  The 2-factor MFAPM only contains the real personal consumption growth and the capital share growth as shown in Figure \ref{fig:2-factor}. The prior means of betas in the simplified 2-factor MFAPM are all significant from zero.
\begin{figure}[H]
    \centering
    \includegraphics[width=1\textwidth]{figures/9-factorbetapriors.jpg}
    \caption{Beta Priors: 9-Factor MFAPM }
    \label{fig:9-factor}
\end{figure}
\begin{figure}[H]
    \centering
    \includegraphics[width=1\textwidth]{figures/10-factorbetapriors.jpg}
    \caption{Beta Priors: 10-Factor MFAPM }
    \label{fig:10-factor}
\end{figure}
\begin{figure}[H]
    \centering
    \includegraphics[width=1\textwidth]{figures/2-factorbetapriors.jpg}
    \caption{Beta Priors: 2-Factor MFAPM }
    \label{fig:2-factor}
\end{figure}
\smallbreak
Figure \ref{fig:9-factor} plots the beta prior means of 9-factor MFAPM estimated by \cite{bianchi2017macroeconomic}; Figure \ref{fig:10-factor} plots the new 10-factor MFAPM including 9 factors proposed by \cite{bianchi2017macroeconomic} and the capital share growth factor proposed by \cite{lettau2019capital}. For the sake of comparison, this paper also plots the prior means of a simplified 2-factor MFAPM betas in Figure \ref{fig:2-factor}. Prior means of betas are calculated by equation (\ref{eq:mfapm}) using the first 10 years sample: data from 1972Q1 to 1981Q4. According to Figure \ref{fig:9-factor}, among all portfolios, most of 9-factor MFAPM betas are insignificant from zero: only betas of the rate of real personal consumption growth, the 1-month real T-bill return, and the Bond premium factor are not centered at zero. In Figure \ref{fig:10-factor}, the prior mean of capital share growth beta is significant from zero among most portfolios, while most prior means of other factor betas are close to zero, same as shown by Figure \ref{fig:9-factor}. Risk premiums estimated by \cite{bianchi2017macroeconomic} using B-TVB-SV model supports the assumption that only a small friction of factors are significant: among all 9 factors, only risk premiums of excess return of a value weighted market portfolio, the industrial production, the unexpected inflation rate and the Liquidity factor are significant from zero. 
\smallbreak
The inconsistency between factor set with non-zero beta prior mean and factor set with non-zero risk premiums rises another question: is model misspecification problem solved by the B-TVB-SV frame work? The B-TVB-SV model estimates F-MB two stages in each iteration. Under the B-TVB-SV framework, the sampling process of risk premiums is designed as follows: risk premiums are assumed to follow an multi-variate distribution, and estimation error ($\tau^2$ in equation (\ref{eq:btvbsv2})) is assumed to follow an inverse Gamma-2 distribution. Variance $\tau^2$ is updated conditional on estimated factor loadings from first stage, and the risk premiums are then updated conditional the state variance. The standard error of risk premiums estimated by F-MB is biased when autocorrelation present within factors. As the drawbacks of F-MB approach pointed out by \cite{jagannathan1998asymptotic}, when the first step regression is misspecified, the second step might generate significant premiums incorrectly. The updating of first-stage beta in B-TVB-SV approach does not rely on the second-stage estimated values of $\lambda$s. The beta are updated only conditional on the portfolio return volatility and breaks in idiosyncratic risks. Therefore, the sampling process cannot guarantee that the model captures the true DGP: although two stages are linked by volatility of factor loadings, the robustness of risk premiums estimation is still conditional on that the model is correctly specified.
\smallbreak
To maintain the robustness of model specification, this paper makes the following assumption: the true beta matrix is assumed to be a sparse matrix only containing a few non-zero elements. Basing on this assumption, this paper propose an alternative model for the original B-TVB-SV: according to the theoretical justification provided by \cite{lettau2019capital}, the real consumption growth and capital share growth are considered as "core" factors, while all factors other than "core" factors are considered as "redundant" factors in the MFAPM model. The alternative model assumes the true factor loadings and risk premiums for "redundant" factors are both insignificant from zero. However, the alternative model cannot simply exclude all "redundant" factors and only estimate "core" factors. The capital share growth is biased itself. Firstly, capital share growth as a risk factor is subject to measurement error problem. Pre-existing literatures have pointed out that measurement errors are caused by smoothing-type filters used during the construction of macroeconomics data, and motivated the use of long-horizon data in asset pricing estimations (see \cite{daniel1997equity}, \cite{parker2005consumption}, and \cite{kroencke2017asset}). Long-horizon capital share growth is used by \cite{lettau2019capital} to tackle the potential measurement error problem. Secondly, another reason for using long-horizon capital share growth is to avoid the misspecification of SDF \citep{lettau2019capital}. The SDF in equation (\ref{eq:ks_apx}) contains an error term $\mu_t$, which indicates that a MFAPM only containing core factors is actually an approximation of the true data generation process (DGP), and thus is highly likely to be misspecified. 
\smallbreak
 Based upon the 9-factor MFAPM model estimated by \cite{bianchi2017macroeconomic}, the alternative MFAPM includes 10 factors and different prior setting. In the alternative model, the monthly real consumption growth and the monthly capital share growth are both included as core risk factors. Priors adopted for core factors are flat prior, which is very informative. Additionally, "redundant" factors \footnote{8 factors from the 9-factor MFAPM: the excess return of a value weighted market portfolio, the default risk premium change, the unexpected inflation rate, the change in term premium, the industrial production, the 1-month real T-bill return, Liquidity factor and the Bond premium factor.} with shrinkage priors are included in order to cancel out the effect of measurement error and avoid model misspecification problem.
\input{chapters/shrinkage/savs.tex}


==> chapters/static_f-mb.tex <==
Within each iteration, the first step of F-MB bootstrap approach is based upon ICAPM theories: a time-series analysis using equation (\ref{eq:mfapm}) to estimate risk loadings (betas) for individual factors. The second step is based upon APT: a cross-sectional regression using no-arbitrage condition to obtain factor risk premiums. Under no-arbitrage condition, equation (\ref{eq:ereturn}) and equation (\ref{eq:b}) hold \citep{cochrane2009asset}:
\begin{equation}
    E_t(r_{i,t+1})=\frac{cov_t(F_{t+1},r_{i,t+1})}{cov_t(F_{t+1},F'_{t+1})}\times-r^f_t cov_t(F_{t+1},\Tilde{F}_{t+1})
    \label{eq:ereturn}
\end{equation}
\begin{equation}
    b_t=\beta'_{i,t}\lambda_t
    \label{eq:b}
\end{equation}
where $\Tilde{F}_t$ denotes $(1, F_t)$ which is a vector containing a constant number one and all factors; $\beta_t=(\beta_{1,t},...,\beta_{K,t})$ is the coefficient vector of factors in SDF; $\lambda_t$ denotes the vector of factor risk premiums.
 
Therefore, the second step cross-sectional regression is as follows:
\begin{equation}
    r_{i,t}=\lambda_{0,t}+\sum^ K_{j=1}\lambda_{j,t}\hat{\beta}_{ij,t}+\zeta_{i,t}~~~~~~~~~~~\zeta_{i,t}\sim N(0,\tau^2)
    \label{eq:2nd_step}
\end{equation}
where $\hat{\beta}_{ij,t}$ are risk loadings obtained from the first step.  The standard errors of risk premiums $\lambda_{j,t}$ are calculated using estimated risk premiums and robust to cross-sectional correlation. Therefore, the F-MB bootstrap approach corrects the standard errors of risk premiums caused by the comovement of factors within each iteration.%The cross-sectional regression is also a test of the pricing power of risk factors: the pricing error $\lambda_{0,t}$ is zero if there is no price anomalies. 

%However, the static F-MB approach for estimating risk premiums only takes cross-sectional correlation into consideration, but fails to capture firm effect\footnote{The idiosyncratic risk of a given firm may be correlated across years.} across time \citep{petersen2009estimating}. 


